TNT: Text-Conditioned Network with Transductive Inference for Few-Shot Video Classification

Recently, few-shot video classification has received an increasing interest. Current approaches mostly focus on effectively exploiting the temporal dimension in videos to improve learning under low data regimes. However, most works have largely ignored that videos are often accompanied by rich textual descriptions that can also be an essential source of information to handle few-shot recognition cases. In this paper, we propose to leverage these human-provided textual descriptions as privileged information when training a few-shot video classification model. Specifically, we formulate a text-based task conditioner to adapt video features to the few-shot learning task. Furthermore, our model follows a transductive setting to improve the task-adaptation ability of the model by using the support textual descriptions and query instances to update a set of class prototypes. Our model achieves state-of-the-art performance on four challenging benchmarks commonly used to evaluate few-shot video action classification models.

==> text/results_rebuttal_version.tex <==
% \begin{table}[t]
% \caption{\textbf{Dataset statistics}, using the evaluation protocol of~\cite{Cao_2020_TAM,compoundMem} in Kinetics~\cite{kinetics} and Something-Something-V2~\cite{S2Sv2Goyal}, respectively termed as Kinetics-100 and SS-100.} %title of the table
% \centering % centering table
% \resizebox{8.3cm}{!}{%
%     \begin{tabular}{cccccccc} % creating eight columns
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{\bf Dataset}} &\multicolumn{3}{c}{\bf Num Classes} & \multicolumn{3}{c}{\bf Num Instances} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}{\bf Textual} \\ {\bf Descriptions} \end{tabular}}} \\
%     \cmidrule{2-7}
%     % \cmidrule{2-4} & \cmidrule{5-7} 
%          & Train & Val & Test & Train & Val & Test & \\
%     \midrule
        
%     Kinetics-100 & 64 & 12 & 24 & 6400 & 1200 & 2400 & class level
%     \\
%     SS-100 & 64 & 12 & 24 & 67013 & 1926 & 2857 & video level
%     \\
%     \bottomrule
%     \end{tabular}}
% \label{tab:datasets}
% \end{table}

% \begin{table*}[!b]
% \caption{\textbf{Few-Shot classification results.} For all reported methods, we show Top-1 accuracy on the meta-testing sets of Kinetics-100 and SS-100 for the 5-way 1-shot and 5-way 5-shot tasks.} %title of the table
% \centering % centering table
% \vspace{-10pt}
% \resizebox{14.0cm}{!}{%
%     \begin{tabular}{cccccc} % creating eight columns
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{\bf Model}} & \multicolumn{2}{c}{\bf Kinetics-100} & \multicolumn{2}{c}{\bf SS-100} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\bf Backbone \end{tabular}}}
%     \\\cmidrule{2-5} 
%          & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} &  \\
%     \midrule
%     Matching Networks~\cite{compoundMem} & 53.3 & 74.6 & - & - & \multirow{7}{*}{\begin{tabular}[c]{@{}c@{}} ResNet 50 \end{tabular}}
%     \\
%     MAML~\cite{compoundMem} & 54.2 & 75.3 & - & - &
%     \\
%     CMN~\cite{compoundMem} & 60.5 & 78.9 & - & - &
%     \\ % Entering row contents
%     TSN++~\cite{Cao_2020_TAM} & 64.5 & 77.9 & 33.6 & 43.0 &
%     \\
%     CMN++~\cite{Cao_2020_TAM} & 65.4 & 78.8 & 34.4 & 43.8 &
%     \\
%     TRN++~\cite{Cao_2020_TAM} & 68.4 & 82.0 & 38.6 & 48.9 &
%     \\
%     TAM~\cite{Cao_2020_TAM} & 73.0 & \textbf{85.8} & 42.8 & 52.3 &
%     %\\
%     %\hline
%     %\begin{tabular}[c]{@{}c@{}}TNT \end{tabular} & \begin{tabular}[c]{@{}c@{}}76.40 \\ \pm 0.22 \end{tabular} & %\begin{tabular}[c]{@{}c@{}}84.74 \\ \pm 0.19 \end{tabular} & \begin{tabular}[c]{@{}c@{}}44.43 \\ \pm 0.24 \end{tabular} & %\begin{tabular}[c]{@{}c@{}}53.50 \\ \pm 0.24 \end{tabular} &  \begin{tabular}[c]{@{}c@{}} ResNet \\ 50 \end{tabular}
%     \\
%     % \hline
%     %\begin{tabular}[c]{@{}c@{}}TNT \end{tabular} & \begin{tabular}[c]{@{}c@{}}74.92 \\ \pm 0.24 \end{tabular} & \begin{tabular}[c]{@{}c@{}}84.14 \\ \pm 0.17 \end{tabular} & \begin{tabular}[c]{@{}c@{}}43.17 \\ \pm 0.19 \end{tabular} & \begin{tabular}[c]{@{}c@{}}51.43 \\ \pm 0.19 \end{tabular} &  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} ResNet \\ 34 \end{tabular}}
%     %\\
%     \cmidrule{1-6} 
%     % \hline
%     \begin{tabular}[c]{@{}c@{}}TNT \end{tabular}& \begin{tabular}[c]{@{}c@{}}\textbf{76.51} \pm 0.23 \end{tabular} & \begin{tabular}[c]{@{}c@{}}83.40 \pm 0.18  \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{50.20} \pm 0.21 \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{58.46} \pm 0.19 \end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}} ResNet 34 \end{tabular}
%     \\
%     \bottomrule
%     \end{tabular}
% }
% \vspace{-10pt}
% \label{tab:main_results}
% \end{table*}

\noindent\textbf{Datasets.}
We evaluate our approach using two families of datasets: (i) those with rich and detailed textual descriptions of actions per video: Epic-Kitchens~\cite{epickitchens}, Something-Something-V2~\cite{S2Sv2Goyal}, and (ii) those with short class-level descriptions: UCF-101~\cite{DBLP:journals/corr/abs-1212-0402} and Kinetics~\cite{kinetics}. We propose for the first time to use Epic-Kitchens~\cite{epickitchens} as a benchmark for few-shot video classification. We coin this new benchmark \textbf{Epic-Kitchens-92} (EK-92). \cite{epickitchens} features spontaneous actions accompanied with human narrations. Interestingly, a particular action class could encompass diverse narrations,~\eg, the action class: ``\textit{\underline{Put} something}" features narrations such as: ``\textit{\underline{Put}
plate \underline{down}}", ``\textit{\underline{Place} aubergine \underline{onto} pan}". To ensure that action classes are consistent, we use the 97 verb classes defined by~\cite{epickitchens} and select those with more than 5 instances, yielding 92 action classes. Then, we divide the resulting 92 classes into 58, 11, and 23 for meta-training, meta-validation, and meta-testing, respectively.
For the other benchmarks, we follow the evaluation protocol proposed by \cite{Cao_2020_TAM, mishra2018generative,compoundMem} termed  \textbf{Something-Something-100} (SS-100), \textbf{MetaUCF-101}, and \textbf{Kinetics-100}, respectively.
The protocols in \cite{Cao_2020_TAM,compoundMem} define a set of 64 classes for meta-training, 12 classes for meta-validation, and 24 classes for meta-testing, which are sampled randomly from Something-Something-V2 and Kinetics, respectively. In terms of the protocol in \cite{mishra2018generative}, it samples randomly 70 classes from UCF-101 for meta-training, 10 classes for meta-validation, and 21 for meta-testing. To facilitate the comparison, we use the same partitions proposed by the original authors.

Additionally, we make use of the provided text-based action descriptions from every meta-dataset. 
In Kinetics-100 and MetaUCF-101, we directly employ the class labels (\eg, \textit{Headbanging}, \textit{Stretching leg}, etc), which are the same for all samples that belong to the same class. Alternatively, EK-92 and SS-100 provide a fine-grained textual action description per instance based on the action and objects depicted in the video. 
% Unlike EK-92, SS-100 has structured textual descriptions (\eg, class label: \textit{Approaching \underline{something} with your camera}; instance textual description: \textit{Approaching \underline{\textbf{2 bicycle wheels}} with your camera}).
%We exploit these fine-grained labels as: (i) they usually correlate with the visual information shown in the videos, and (ii) they can be gathered in commercial applications~\eg,~Instagram, TikTok and general personal data management tools.
% Table~\ref{tab:datasets} summarizes the most relevant details of datasets.
Further details about these datasets can be found in the Supplementary Material. 

% We evaluate our approach using four challenging benchmarks for few-shot action recognition, namely Epic-Kitchens \cite{epickitchens}, Something-Something-V2 \cite{S2Sv2Goyal} and UCF-101 \cite{DBLP:journals/corr/abs-1212-0402} and Kinetics~\cite{kinetics}.
% For fair comparison, we follow the evaluation protocol proposed by \cite{Cao_2020_TAM, compoundMem, mishra2018generative} termed  \textbf{Something-Something-100} (SS-100), \textbf{Kinetics-100} and \textbf{MetaUCF-101}, respectively.
% The first two protocols \cite{compoundMem, Cao_2020_TAM} define a set of 64 classes for meta-training, 12 classes for meta-validation, and 24 classes for meta-testing, which were sampled randomly from Kinetics and Something-Something-V2. Conversely, the last one protocol \cite{mishra2018generative} sample randomly from UCF-101 70 classes for meta-training, 10 classes for meta-validation and 21 for meta-testing. 
% We use the exact same partition proposed by the original authors instead of randomly sampling again the specific categories for each meta-dataset.

% Additionally, we also make use of the provided text-based action descriptions from every meta-dataset. 
% In Kinetics-100 and MetaUCF-101, we directly employ the class labels (\eg, \textit{Headbanging}, \textit{Stretching leg}, etc), which are the same for all samples that belong to the same class. Alternatively, SS-100 provides a fine-grained textual action description per instance based on the action label and objects depicted in the video. As an example, for the action label \textit{Approaching \underline{something} with your camera}, it is possible to find a video with the textual action description \textit{Approaching \underline{\textbf{2 bicycle wheels}} with your camera}. We exploit these fine-grained labels as: (i) they usually correlate with the visual information shown in the videos, and (ii) they can be gathered in commercial applications~\eg,~Instagram, TikTok, and general personal data management tools. Table~\ref{tab:datasets} summarizes the most relevant details of each dataset.

% We evaluate our approach in two kinds of datasets: those with a general description by class like Kinetics \cite{kinetics}, UCF101 \cite{ucf101}, and Sports 1M \cite{sports1M}, and those like Something-Something-V2 \cite{S2S-V2Goyal} and Epic Kitchens \cite{epickitchens} which have a fine-grained and very correlated description for each video.

% In this regard, we select two datasets from these groups: Kinetics \cite{kinetics}, ans Something-Something-V2 \cite{S2S-V2Goyal}. These datasets are used in previous researches. However, the last one has not been explored before in this area and proposes an interesting setup. It has some classes with very few examples, thus simulating a real few-shot learning scenario. Moreover, it includes video descriptions that can be different in verbs or objects between elements of the same class.

% For Kinetics \cite{kinetics} and Something-Something-V2 \cite{S2S-V2Goyal}, we follow the same splits as \cite{compoundMem} and \cite{Cao_2020_TAM}, respectively, for a fair comparison. These splits contain 64 classes for meta-training, 12 classes for meta-validation, and 24 classes for meta-testing, which were sampled randomly from the full dataset. Furthermore, we add the action descriptions to every meta-dataset; for Kinetics \cite{kinetics}, we employ the class labels, which are generals and the same to all samples that belong to the same class. Alternatively, Something-Something-V2 \cite{S2S-V2Goyal} provides different labels by samples based on the class label and the action objects, e.g., Class label: Approaching something with your camera, Action description: Approaching \textbf{2 bicycle wheels} with your camera. Because these labels are very correlated to the visual information shown in the corresponding videos, we select them to describe each video.

% \andres{Write about epic kitchens}

% - We evaluate our model in two kinds of dataset: those that have a genaral descriptions by class like Kinetics, UCF101 and Sports 1M, and those like S2S-V2 and Epic kitchens which have a fine grained description for each video, and these actions descriptions and the action videos are very correlected. 

% - To evaluate the performance of our model in these kind of datasets, we select the kinetics, Something-Something-V2, which are used on previus research, and Epic Kitchens. Este ultimo dataset no ha sido explorado antes en esta area y propone una configuración muy interesante, donde existen algunas clases que tienen muy poco ejemplos, simulando así un escenario real de few-shot learning. Además, incluye descripciones detalladas por videos, las cuales pueden ser diferentes en verbo u objetos entre elementos de la misma clase.

% - For Kinetics and Something-Something-V2, we follow the same splits as \cite{compoundMem} and \cite{Cao_2020_TAM}, respectively for a fair comparison. These splits contain 64 classes for meta-training, 12 classes for meta-validation and 24 classes for meta-testing, which were sampled ramdomly from the fully dataset. 

% - Furthermore, we add the action description to each video, for Kinetics we employ the action labels which are generals and the same to all samples that belong to the same class. Alternatively, Something-Something-V2 has disjoint labels between samples, these labels are (poner ejemplo que se diferencian entre elementos de una misma clase por el objeto al que hacen referencia) 

\setboolean{main_document}{false}   
\ifthenelse{\boolean{main_document}}{
\begin{table}[t]

% \caption{\textbf{Dataset statistics}, using the evaluation protocol of~\cite{Cao_2020_TAM,mishra2018generative,compoundMem} in Something-Something-V2~\cite{S2Sv2Goyal}, UCF-101 \cite{DBLP:journals/corr/abs-1212-0402} and Kinetics~\cite{kinetics}, respectively termed as SS-100, MetaUCF-101 and Kinetics-100. We also introduce EK-92, a new data split for Epic-Kitchens \cite{epickitchens}}

%title of the table
\centering % centering table
\resizebox{8.3cm}{!}{%
    \begin{tabular}{cccccccc} % creating eight columns
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\bf Dataset}} &\multicolumn{3}{c}{\bf Num Classes} & \multicolumn{3}{c}{\bf Num Instances} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}{\bf Rich Textual} \\ {\bf Descriptions} \end{tabular}}} \\
    \cmidrule{2-7}
    % \cmidrule{2-4} & \cmidrule{5-7} 
         & Train & Val & Test & Train & Val & Test & \\
    \midrule
    EK-92 & 58 & 11 & 23 & 49621 & 8352 & 18370 & \cmark  
    \\
    SS-100 & 64 & 12 & 24 & 67013 & 1926 & 2857 & \cmark
    \\
    MetaUCF-101 & 70 & 10 & 21 & 9154 & 1421 & 2745 & \xmark
    \\
    Kinetics-100 & 64 & 12 & 24 & 6400 & 1200 & 2400 & \xmark
    \\
    \bottomrule
    \end{tabular}}
\caption{Statistics from the SS-100~\cite{Cao_2020_TAM}, MetaUCF-101~\cite{mishra2018generative}, and Kinetics-100~\cite{compoundMem} datasets for FSL. We introduce EK-92, a new data split from Epic-Kitchens~\cite{epickitchens}.}
\label{tab:datasets}
\end{table}
}{}
% \begin{table*}[!b]
% \caption{\textbf{Few-Shot classification results.} For all reported methods, we show Top-1 accuracy on the meta-testing sets of EK-92, SS-100, UCF-101 and Kinetics-100 for the 5-way 1-shot and 5-way 5-shot tasks.} %title of the table
% \centering % centering table
% \vspace{-10pt}
% \resizebox{14.0cm}{!}{%
%     \begin{tabular}{cccccccccc} % creating eight columns
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{\bf Model}} & \multicolumn{2}{c}{\bf Kinetics-100} & \multicolumn{2}{c}{\bf SS-100} & \multicolumn{2}{c}{\bf EK-92} & \multicolumn{2}{c}{\bf MetaUCF-101} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\bf Backbone \end{tabular}}}
%     \\\cmidrule{2-9} 
%          & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & 
%          \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \\
%     \midrule
%     % Matching Networks~\cite{compoundMem} & 53.3 & 74.6 & - & - & - & - & - & - & \multirow{7}{*}{\begin{tabular}[c]{@{}c@{}} ResNet 50 \end{tabular}}
%     % \\
%     % MAML~\cite{compoundMem} & 54.2 & 75.3 & - & - & - & - & - & - &
%     % \\
%     % CMN~\cite{compoundMem} & 60.5 & 78.9 & - & - & - & - & - & - &
%     % \\ % Entering row contents
%     TSN++~\cite{Cao_2020_TAM} & 64.5 & 77.9 & 33.6 & 43.0 & - & - & - & - &
%     \\
%     CMN++~\cite{Cao_2020_TAM} & 65.4 & 78.8 & 34.4 & 43.8 & - & - & - & - &
%     \\
%     TRN++~\cite{Cao_2020_TAM} & 68.4 & 82.0 & 38.6 & 48.9 & - & - & - & - &
%     \\
%     TAM~\cite{Cao_2020_TAM} & 73.0 & \textbf{85.8} & 42.8 & 52.3 & - & - & - & - &
%     %\\
%     %\hline
%     %\begin{tabular}[c]{@{}c@{}}TNT \end{tabular} & \begin{tabular}[c]{@{}c@{}}76.40 \\ \pm 0.22 \end{tabular} & %\begin{tabular}[c]{@{}c@{}}84.74 \\ \pm 0.19 \end{tabular} & \begin{tabular}[c]{@{}c@{}}44.43 \\ \pm 0.24 \end{tabular} & %\begin{tabular}[c]{@{}c@{}}53.50 \\ \pm 0.24 \end{tabular} &  \begin{tabular}[c]{@{}c@{}} ResNet \\ 50 \end{tabular}
%     \\
%     % \hline
%     %\begin{tabular}[c]{@{}c@{}}TNT \end{tabular} & \begin{tabular}[c]{@{}c@{}}74.92 \\ \pm 0.24 \end{tabular} & \begin{tabular}[c]{@{}c@{}}84.14 \\ \pm 0.17 \end{tabular} & \begin{tabular}[c]{@{}c@{}}43.17 \\ \pm 0.19 \end{tabular} & \begin{tabular}[c]{@{}c@{}}51.43 \\ \pm 0.19 \end{tabular} &  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} ResNet \\ 34 \end{tabular}}
%     %\\
%     \cmidrule{1-10} 
%     ARN \cite{zhang2020fewshot} & 63.7 & 82.4 & - & - & - & - & 62.1 & 84.8 & C3D
%     \\
%     \cmidrule{1-10} 
%     TSN++ Transductive & 66.7 & 78.3 & 32.7 & 50.4 & 38.36 & 49.94 & 77.67 & 85.61 & ResNet 34
%     \\
%     TSN++ Transductive & 68.0 & 79.87 & 35.72 & 47.80 & -- & 52.66 & 79.23 & 90.08 & ResNet 50
%     \\
%     \cmidrule{1-10} 
%     % \hline
%     \begin{tabular}[c]{@{}c@{}}TNT \end{tabular}& \begin{tabular}[c]{@{}c@{}}\textbf{76.51} \pm 0.23 \end{tabular} & \begin{tabular}[c]{@{}c@{}}84.40 \pm 0.18  \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{50.20} \pm 0.21 \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{58.46} \pm 0.19 \end{tabular} & \textbf{42.50} \pm 0.21 & \textbf{57.78} \pm 0.18 & \textbf{85.66} \pm 0.18 & \textbf{92.90} \pm 0.10 &
%     \begin{tabular}[c]{@{}c@{}} ResNet 34 \end{tabular}
%     \\
%     % \hline
%     \begin{tabular}[c]{@{}c@{}}TNT \end{tabular}& \textbf{78.02} \pm 0.24 & \begin{tabular}[c]{@{}c@{}}84.82 \pm 0.19  \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{50.44} \pm 0.25 \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{59.04} \pm 0.23 \end{tabular} & -- & -- & \textbf{86.66} \pm 0.19 & \textbf{94.14} \pm 0.11 &
%     \begin{tabular}[c]{@{}c@{}} ResNet 50 \end{tabular}
%     \\
%     \bottomrule
%     \end{tabular}
% }
% \vspace{-10pt}
% \label{tab:main_results}
% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% COMPLETE CVPR VERSION %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[!b]
% \caption{\textbf{Few-Shot classification results.} For all reported methods, we show Top-1 accuracy on the meta-testing sets of EK-92, SS-100, UCF-101 and Kinetics-100 for the 5-way 1-shot and 5-way 5-shot tasks.} %title of the table
% \centering % centering table
% \vspace{-10pt}
% \resizebox{16.0cm}{!}{%
%     \begin{tabular}{cccccccccc} % creating eight columns
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{\bf Model}} & \multicolumn{2}{c}{\bf EK-92} & \multicolumn{2}{c}{\bf SS-100} & \multicolumn{2}{c}{\bf MetaUCF-101} & \multicolumn{2}{c}{\bf Kinetics-100} & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\bf Backbone \end{tabular}}}
%     \\\cmidrule{2-9} 
%          & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & 
%          \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \\
%     \midrule
%     Matching Networks~\cite{compoundMem} & - & - & - & - & - & - & 53.3 & 74.6 & \multirow{7}{*}{\begin{tabular}[c]{@{}c@{}} ResNet 50 \end{tabular}}
%     \\
%     MAML~\cite{compoundMem} & - & - & - & - & - & - & 54.2 & 75.3 &
%     \\
%     CMN~\cite{compoundMem} & - & - & - & - & - & - & 60.5 & 78.9 &
%     \\ % Entering row contents
%     TSN++~\cite{Cao_2020_TAM} & 39.1 & 52.3 & 33.6 & 43.0 & 76.4 & 88.5 & 64.5 & 77.9 &
%     \\
%     CMN++~\cite{Cao_2020_TAM} & - & - & 34.4 & 43.8 & - & - & 65.4 & 78.8 &
%     \\
%     TRN++~\cite{Cao_2020_TAM} & - & - & 38.6 & 48.9 & - & - & 68.4 & 82.0 &
%     \\
%     TAM~\cite{Cao_2020_TAM} & - & - & 42.8 & 52.3 & - & - & 73.0 & \textbf{85.8} &
%     %\\
%     %\hline
%     %\begin{tabular}[c]{@{}c@{}}TNT \end{tabular} & \begin{tabular}[c]{@{}c@{}}76.40 \\ \pm 0.22 \end{tabular} & %\begin{tabular}[c]{@{}c@{}}84.74 \\ \pm 0.19 \end{tabular} & \begin{tabular}[c]{@{}c@{}}44.43 \\ \pm 0.24 \end{tabular} & %\begin{tabular}[c]{@{}c@{}}53.50 \\ \pm 0.24 \end{tabular} &  \begin{tabular}[c]{@{}c@{}} ResNet \\ 50 \end{tabular}
%     \\
%     % \hline
%     %\begin{tabular}[c]{@{}c@{}}TNT \end{tabular} & \begin{tabular}[c]{@{}c@{}}74.92 \\ \pm 0.24 \end{tabular} & \begin{tabular}[c]{@{}c@{}}84.14 \\ \pm 0.17 \end{tabular} & \begin{tabular}[c]{@{}c@{}}43.17 \\ \pm 0.19 \end{tabular} & \begin{tabular}[c]{@{}c@{}}51.43 \\ \pm 0.19 \end{tabular} &  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} ResNet \\ 34 \end{tabular}}
%     %\\
%     \cmidrule{1-10} 
%     ARN \cite{zhang2020fewshot} & - & - & - & - & 62.1 & 84.8 & 63.7 & 82.4 & C3D
%     \\
%     \cmidrule{1-10} 
%     TSN++ Transductive & 38.36 & 49.94 & 32.7 & 50.4 & 77.67 & 85.61 & 66.7 & 78.3 & ResNet 34
%     \\
%     TSN++ Transductive & 42.33 & 52.66 & 39.28 & 52.63 & 79.23 & 90.08 & 68.0 & 79.87 & ResNet 50
%     \\
%     \cmidrule{1-10} 
%     % \hline
%     TNT & \textbf{42.50} \pm 0.21 & \textbf{57.78} \pm 0.18 & \textbf{50.20} \pm 0.21 & \textbf{58.46} \pm 0.19 & \textbf{85.66} \pm 0.18 & \textbf{92.90} \pm 0.10 & \textbf{76.51} \pm 0.23 & 84.40 \pm 0.18 &
%     ResNet 34
%     \\
%     % \hline
%     TNT & \textbf{46.13} \pm 0.27 & \textbf{59.00} \pm 0.23 & \textbf{50.44} \pm 0.25 & \textbf{59.04} \pm 0.23 & \textbf{86.66} \pm 0.19 & \textbf{94.14} \pm 0.11 & \textbf{78.02} \pm 0.24 & 84.82 \pm 0.19 & ResNet 50
%     \\
%     \bottomrule
%     \end{tabular}
% }
% \vspace{-10pt}
% \label{tab:main_results}
% \end{table*}

\noindent\textbf{Implementation Details.}
We train our model following the episodic learning approach to mimic the meta-testing conditions \cite{8578229}.
For this purpose, we assemble $N$-way and $K$-shot tasks, selecting $N$ classes randomly with $K$ samples for the support set and $B$ unlabeled samples for the query set. Thus, each episode has $NK+B$ videos. We report results for the 5-shot and 1-shot tasks, each with 5-ways and 50 elements of these classes in the query set (10 elements per class). 
% During the evaluation, the sampled query set is built with 10 samples per class which are also used during the transductive inference step.
Our model was trained during $15\times10^{3}$ episodes with the same data augmentation proposed in \cite{TSN}, using $T=8$ frames per video. 
% Each frame is resized to $256\times256$ and then randomly cropped into $224\times224$ images.  
We calculate the mean accuracy by sampling $10^{4}$ episodes (for a total of $5\times10^{5}$ queries) to test our model.
%During training, our model is evaluated every $100$ episodes. 
In regards to the FiLM generator and the distance module, we follow the design choices in~\cite{BateniSimpleCNAPS}. We optimize our model using task batch size of $16$ and Adam with a learning rate of $5\times 10^{-4}$ for EK-92, SS-100 and MetaUCF-101, and $1\times 10^{-4}$ for Kinetics-100.

For our feature encoder, we use a TSN Network with a ResNet-50 backbone pre-trained on ImageNet and augmented with FiLM layers. For the first training stage of the TSN backbone, we tune it during 12 epochs using the setting proposed in \cite{TSN}. 
% We implement the whole model by using the PyTorch framework~\cite{pytorch}. 

% For our feature encoder, we use a TSN Network \cite{TSN} with a ResNet-50 \cite{He_2016_CVPR} backbone, following \cite{Cao_2020_TAM}. 
% % Furthermore, we employ a ResNet-34 \cite{He_2016_CVPR} to analyze our model performance with fewer parameters. 
% We augment the model with FiLM layers. We start our training strategy from ImageNet initialization. % or be previously trained in the meta-training set in a fully supervised way. 
% For the first training stage of the TSN backbone, we tune it during 12 epochs using the setting proposed by \cite{TSN}. %, and a learning rate of 0.01 for SS-100 and MetaUCF101 and 0.001 for Kinetics-100. 
% We implement the whole model by using the PyTorch framework~\cite{pytorch}. %The entire model was trained for 40 hours on 3 and 1 Titan RTX-2080 for the versions with ResNet-50 and ResNet-34, respectively.

% For our feature encoder, we use a TSN Network \cite{TSN} with a ResNet-34 \cite{He_2016_CVPR} as a backbone. We augment the model with FiLM layers. We start our training strategy from ImageNet initialization. % or be previously trained in the meta-training set in a fully supervised way. 
% For the first training stage of the TSN backbone, we tune during 12 epochs using the setting proposed by \cite{TSN}. %, and a learning rate of 0.01 and 0.001 for SS-100 and Kinetics-100, respectively. 
% We implement the whole model with NumPY and PyTorch framework~\cite{harris2020array,pytorch}. The full model was trained and tested on a Titan RTX-2080 for 40 hours.

% We train our model following the episodic learning approach to mimic the data scarcity that the model has to deal with in test time \cite{8578229}. For this purpose, we assemble $N$-way and $K$-shot tasks, selecting $N$ classes randomly with $K$ samples for the support set and $B$ unlabeled samples for the query set. Thus, each episode has $N(K+B)$ videos. We report results for the 5-shot and 1-shot tasks, each one with 5-ways and 10 elements by class in the query set. 

% Our model was trained during $15000$ episodes with the same data augmentation proposed in \cite{TSN} and $8$ frames per video sampled following the protocol described in \cite{TSN}.  We calculate the mean accuracy by randomly sampling $200$ and $10000$ episodes to evaluate and test our model, respectively. The model is evaluated every $100$ episodes. We design our model based on the Simple CNAPS model \cite{BateniSimpleCNAPS}, so we use the same configuration as \cite{BateniSimpleCNAPS}. We optimize our model using Adam with a learning rate of $5\times 10^{-4}$ and $16$ tasks by batch.

% For our feature encoder, we use a TSN Network \cite{TSN} with a ResNet-34 \cite{He_2016_CVPR} as a backbone, augmented with a FiLM layer. This network can be initialized with ImageNet or be previously trained in the meta-training set in a fully supervised way. To do that, we train the TSN during 12 epoch using the setting proposed by [3], and a learning rate of 0.01 and 0.001 for S2S-V2 and Kinetics, respectively. 

% For our feature encoder, we use a TSN Network \cite{TSN} with a ResNet-34 \cite{He_2016_CVPR} as a backbone, augmented with a FiLM layer. 
% This network is initialized with ImageNet pre-trained.\andres{incluir preentrenado en las clases bases} 
% To compute the action descriptions embeddings, we use a pre-trained RoBERTa for sentence representation \cite{reimers2019sentencebert}. Both RoBERTa and TSN networks are fixed during meta-training. The other parts of our models come from scratch.
% We implement the whole method on the PyTorch \cite{pytorch} framework. The full model was trained and tested on a TitanRTX 2080 for 40 hours.

% - We train our model following the episodic learning approach to mimic the N-way and K-shot Task, which is the addressed problem. 

% - For this purporse, we select randomly N classes, (de estas) K samples for the support set and B para el query set. Thus, each episode has N(K+B) videos. We report results for the 5-shot and 1-shot tasks each one with 5-ways and 10 samples by class in the query set. 

% - Our model was trained during 15000 episodes with the same data augmentation and sampling strategies proposed by \cite{TSN}. We sample 8 frames for each samples. 

% - We design our model based on the Simple CNAPS model, so that we use the same configuration. We optimize our model using SGD, lr = 5e-4 and a bATCH SIZE = 16. 

% - For our feature encoder, we use a TSN Network with a ResNet-34 backbone augmented with film layer after every ResNet block. This network is initialized with ImageNet pretrained. The Textual Task Encoder has a Roberta pretrained following the approach introduced in \cite{reimers2019sentencebert}. During meta-training these parts are fixed. The other parts of our model come from scratch.

% - We implement the whole method on PyTorch framework. The full model was trained on a TitanRTX 2080 during 50 hours.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% COMPLETE ICCV VERSION %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% datasets with fine grained descriptions %%%%%%%%%%%%

% \begin{table}[t]
% \centering
% \resizebox{13cm}{!}{
% \begin{tabular}{cc}
% \bmvaHangBox{
% \begin{tabular}{ccccc} % creating eight columns
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{\bf Model}} & \multicolumn{2}{c}{\bf EK-92} & \multicolumn{2}{c}{\bf SS-100} 
%     \\\cmidrule{2-5} 
%          & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} \\
%     \midrule
%     TSN++~\cite{Cao_2020_TAM} & $39.1^*$ & $52.3^*$ & $33.6$ & $43.0$
%     \\
%     CMN++~\cite{compoundMem,Cao_2020_TAM} & - & - & 34.4 & 43.8 
%     \\
%     TRN++~\cite{Cao_2020_TAM} & - & - & 38.6 & 48.9  
%     \\
%     TAM~\cite{Cao_2020_TAM} & - & - & 42.8 & 52.3 
%     \\
%     \cmidrule{1-5} 
%     TSN++ Transd. \cite{liu2020prototype} & 42.33 & 52.66 & 39.28 & 52.63 
%     \\
%     % \hline
%     TNT & $\textbf{46.13} \pm 0.27$ & $\textbf{59.00} \pm 0.23$ & $\textbf{50.44} \pm 0.25$ & $\textbf{59.04} \pm 0.23$
%     \\
%     \bottomrule
%     \end{tabular}
% } & \bmvaHangBox{
% \begin{tabular}{ccccc} % creating eight columns
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{\bf Model}} &  \multicolumn{2}{c}{\bf MetaUCF-101} & \multicolumn{2}{c}{\bf Kinetics-100}
%     \\\cmidrule{2-5} 
%          & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} \\
%     \midrule
%     ARN \cite{zhang2020fewshot} & 62.1 & 84.8 & 63.7 & 82.4
%     \\
%     TSN++~\cite{Cao_2020_TAM} & $76.4^*$ & $88.5^*$ & 64.5 & 77.9 
%     \\
%     CMN++~\cite{compoundMem,Cao_2020_TAM} & - & - & 65.4 & 78.8
%     \\
%     TRN++~\cite{Cao_2020_TAM} & - & - & 68.4 & 82.0
%     \\
%     TAM~\cite{Cao_2020_TAM} & - & - & 73.0 & \textbf{85.8}
%     \\
%     \cmidrule{1-5} 
%     TSN++ Transd. \cite{liu2020prototype} & 79.23 & 90.08 & 68.0 & 79.87 
%     \\
%     % \hline
%     TNT & $\textbf{86.66} \pm 0.19$ & $\textbf{94.14} \pm 0.11$ & $\textbf{78.02} \pm 0.24$ & $84.82 \pm 0.19$ 
%     \\
%     \bottomrule
%     \end{tabular}
% }\\(a) & (b)
% \end{tabular}
% }
% \caption{
% \textbf{Results on two families of datasets}. (a) Those with rich textual descriptions, and (b) Those with class-level textual descriptions. We report top-1 accuracy on the meta-testing sets of EK-92 and SS-100 for the 5-way tasks. *Obtained by us.
% }
% \label{tab:datasets_results}
% \end{table}
%%%%%%%%%%%%%% BMVC version %%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\resizebox{13cm}{!}{
\bmvaHangBox{
\begin{tabular}{ccccccccc} % creating eight columns
    \toprule
    \multicolumn{1}{c}{\multirow{3}{*}{\bf Model}} & \multicolumn{4}{c}{\bf with Rich Textual Descriptions} & \multicolumn{4}{c}{\bf with Short Class-Level Description}\\\cmidrule(lr){2-5}\cmidrule(lr){6-9}
    & \multicolumn{2}{c}{\bf EK-92} & \multicolumn{2}{c}{\bf SS-100} & \multicolumn{2}{c}{\bf MetaUCF-101} & \multicolumn{2}{c}{\bf Kinetics-100}
    \\\cmidrule(lr){2-5}\cmidrule(lr){6-9}
         & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} \\
    \midrule
    ARN \cite{zhang2020fewshot} & - & - & - & - & 62.1 & 84.8 & 63.7 & 82.4
    \\
    TSN++~\cite{Cao_2020_TAM} & $39.1^*$ & $52.3^*$ & $33.6$ & $43.0$ & $76.4^*$ & $88.5^*$ & 64.5 & 77.9 
    \\
    CMN++~\cite{compoundMem,Cao_2020_TAM} & - & - & 34.4 & 43.8 & - & - & 65.4 & 78.8
    \\
    TRN++~\cite{Cao_2020_TAM} & - & - & 38.6 & 48.9 & - & - & 68.4 & 82.0
    \\
    TAM~\cite{Cao_2020_TAM} & - & - & 42.8 & 52.3 & - & - & 73.0 & \textbf{85.8}
    \\
    % 3DFSV~\cite{Xian2020GeneralizedMF} & - & - & 59.1 & 80.1 & - & - & 92.5 & 97.8
    % \\
    \cmidrule{1-9} 
    TSN++ Transd. \cite{liu2020prototype} & 42.33 & 52.66 & 39.28 & 52.63 & 79.23 & 90.08 & 68.0 & 79.87 
    \\
    % \hline
    TNT & $\textbf{46.13} \pm 0.27$ & $\textbf{59.00} \pm 0.23$ & $\textbf{50.44} \pm 0.25$ & $\textbf{59.04} \pm 0.23$ & $\textbf{86.66} \pm 0.19$ & $\textbf{94.14} \pm 0.11$ & $\textbf{78.02} \pm 0.24$ & $84.82 \pm 0.19$ 
    \\
    \bottomrule
    \end{tabular}
} 
}
\caption{
\textbf{Results on two families of datasets}. Those with rich textual descriptions: EK-92 and SS-100. Those with class-level textual descriptions: MetaUCF-101 and Kinetics-100. We report top-1 accuracy on the meta-testing sets for the 5-way tasks. *Obtained by us.
}
\vspace{-3mm}
\label{tab:datasets_results}
\end{table}

% \begin{table}[t]
% \caption{\textbf{Results on datasets with rich textual descriptions.} We report top-1 accuracy on the meta-testing sets of EK-92 and SS-100 for the 5-way tasks. *Obtained by us.} %title of the table
% \centering % centering table
% \resizebox{8.3cm}{!}{%
%     \begin{tabular}{ccccc} % creating eight columns
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{\bf Model}} & \multicolumn{2}{c}{\bf EK-92} & \multicolumn{2}{c}{\bf SS-100} 
%     \\\cmidrule{2-5} 
%          & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} \\
%     \midrule
%     TSN++~\cite{Cao_2020_TAM} & $39.1^*$ & $52.3^*$ & $33.6$ & $43.0$
%     \\
%     CMN++~\cite{compoundMem,Cao_2020_TAM} & - & - & 34.4 & 43.8 
%     \\
%     TRN++~\cite{Cao_2020_TAM} & - & - & 38.6 & 48.9  
%     \\
%     TAM~\cite{Cao_2020_TAM} & - & - & 42.8 & 52.3 
%     \\
%     \cmidrule{1-5} 
%     TSN++ Transd. \cite{liu2020prototype} & 42.33 & 52.66 & 39.28 & 52.63 
%     \\
%     % \hline
%     TNT & $\textbf{46.13} \pm 0.27$ & $\textbf{59.00} \pm 0.23$ & $\textbf{50.44} \pm 0.25$ & $\textbf{59.04} \pm 0.23$
%     \\
%     \bottomrule
%     \end{tabular}
% }
% \label{tab:fg_datasets_results}
% \end{table}

% %%%%%%%%%%%%%%%%%%%%%%%% datasets with general descriptions %%%%%%%%%%%%%%%%%%%%%
% \begin{table}[b]
% \caption{\textbf{Results on datasets with class-level descriptions.} We show the top-1 accuracy on MetaUCF-101 and Kinetics-100 for the 5-way tasks. *Obtained by us.} %title of the table
% \centering % centering table
% \resizebox{8.3cm}{!}{%
%     \begin{tabular}{ccccc} % creating eight columns
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{\bf Model}} &  \multicolumn{2}{c}{\bf MetaUCF-101} & \multicolumn{2}{c}{\bf Kinetics-100}
%     \\\cmidrule{2-5} 
%          & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} \\
%     \midrule
%     ARN \cite{zhang2020fewshot} & 62.1 & 84.8 & 63.7 & 82.4
%     \\
%     TSN++~\cite{Cao_2020_TAM} & $76.4^*$ & $88.5^*$ & 64.5 & 77.9 
%     \\
%     CMN++~\cite{compoundMem,Cao_2020_TAM} & - & - & 65.4 & 78.8
%     \\
%     TRN++~\cite{Cao_2020_TAM} & - & - & 68.4 & 82.0
%     \\
%     TAM~\cite{Cao_2020_TAM} & - & - & 73.0 & \textbf{85.8}
%     \\
%     \cmidrule{1-5} 
%     TSN++ Transd. \cite{liu2020prototype} & 79.23 & 90.08 & 68.0 & 79.87 
%     \\
%     % \hline
%     TNT & $\textbf{86.66} \pm 0.19$ & $\textbf{94.14} \pm 0.11$ & $\textbf{78.02} \pm 0.24$ & $84.82 \pm 0.19$ 
%     \\
%     \bottomrule
%     \end{tabular}
% }
% \label{tab:gn_datasets_results}
% \end{table}

\noindent\textbf{Baselines.} We compare the performance of our TNT model against state-of-the-art methods for few-shot video classification, namely TAM \cite{Cao_2020_TAM} and ARN \cite{zhang2020fewshot}. We also consider additional stronger baselines, namely TSN++, TRN++ and CMN++ which are proposed by \cite{Cao_2020_TAM}, following the practices from \cite{chen2020closer, compoundMem}. Because our model makes use of a transductive setting, we also consider a transductive baseline named TSN++ Transd. This baseline is an extension of the image-based method \cite{liu2020prototype} which adopts a pseudo-labeling strategy to augment the support set. Conversely, the method proposed by \cite{Xian2020GeneralizedMF} is not considered because it relies on a large amount of additional data, and its evaluation protocol is different from ours and from the one used in the baselines. Specifically, it uses the whole video instead of a segment of it.
% to overcome the scarce data scenario in a FSL task, therefore, the comparison is not fair. 

\noindent\textbf{Impact of rich textual descriptions.} As it can be observed in Table~\ref{tab:datasets_results}, we achieve state-of-the-art-results in all standard benchmark metrics across the two tested datasets with rich textual descriptions per instance. Notably, our model achieves outstanding results in EK-92, where it must handle spontaneous and unstructured descriptions. Likewise, our model improves over the TSN++ transductive baseline by around 7\% and 4\% in the 5-shot and 1-shot tasks, respectively, which shows the relevance of using the textual descriptions to modulate the network and make a transductive inference. It is worth noting that TSN-based backbone does not have a strong temporal modeling capacity. This is in sharp contrast to TAM~\cite{Cao_2020_TAM}, which is specially designed to capture temporal information. Despite these disadvantages, our method is able to outperform this strong alternative by around 8\% in the 5-shot and 1-shot tasks on SS-100.

\noindent\textbf{Impact of short class-level textual descriptions.} Table~\ref{tab:datasets_results} shows the performance of our model in datasets without rich textual description.  Notably, our model outperforms the state-of-the-art baselines on MetaUCF-101 by a large margin. On Kinetics-100, TNT beats the TAM model, which is the best baseline in this benchmark, in the 1-shot task by 3.5\%, while in the 5-shot, the result remains competitive. A possible reason for such results is that, unlike MetaUCF-101, Kinetics-100 has significantly fewer training instances. These results suggest that TNT achieves outstanding performance with short class-level descriptions, although it is designed to leverage the rich semantic information in fine-grained textual descriptions.

%%%%%% For both CVPR AND ICCV VERSION
% We compare the performance of our full TNT model against three state-of-the-art methods for few-shot video classification, namely TAM \cite{Cao_2020_TAM}, CMN \cite{compoundMem} and ARN \cite{zhang2020fewshot}. 
% Additionally, we compare our method against other baseline methods that are popular in the literature about FSL: Matching Networks~\cite{vinyals2016matching}, MAML~\cite{pmlr-v70-finn17a}, and TSN/TRN++~\cite{chen2020closer}. To make the comparison fairer, we propose a transductive baseline named TSN++ transductive.  This baseline is an extension of the image-based method \cite{liu2020prototype} which adopts a pseudo-labeling strategy to augment the support set. Results are reported in Table~\ref{tab:main_results}.

%%%%%% END first part %%%%%%%

%\paragraph{CMN} 
%\cite{compoundMem} proposes to encode a variable-length video sequence into a multi-saliency embedding function and classify the novel class instances following a compound memory structure similar to \cite{DBLP:journals/corr/KaiserNRB17}. Furthermore,~\cite{compoundMem} implemented two established few-shot image classification methods MAML~\cite{pmlr-v70-finn17a} and Matching Net~\cite{vinyals2016matching}, which were extended for video understanding.

%\paragraph{TAM}~\cite{Cao_2020_TAM} presents a model that explicitly computes the temporal alignment between two video sequences prior to perform the nearest-neighbor classification.
%Based on the findings in~\cite{chen2020closer}, ~\cite{Cao_2020_TAM} also implements stronger baselines for TSN++, CMN++ and TRN++~\cite{TSN,TRNZhou,compoundMem}.

% Our model is compared with TAM \cite{Cao_2020_TAM}, which has state-of-the-art results in FSL for video understanding on Kinetics-100 and SS-100. For a fair comparison, we train and test our method in the same splits that they used and present the same numbers reported by TAM \cite{Cao_2020_TAM}.

%% CVPR VERSION

% As it can be observed in Table~\ref{tab:main_results}, we achieve state-of-the-art-results in 3 out of 4 standard benchmark metrics
% across the two tested datasets. 
% This is significant considering that our backbone is significantly smaller than those of the competing methods.
% Moreover, TSN~\cite{TSN}, our backbone, has only a weak temporal modeling capacity. This is in sharp contrast to TAM~\cite{Cao_2020_TAM} that is specially designed to capture temporal information. Despite these disadvantages, our method is able to outperform strong alternatives and baselines. Critically, on SS-100 our TNT model outperforms the best previous result by around 8\% in the 5-shot and 1-shot tasks. Furthermore, on Kinetics-100, TNT outperforms the TAM model results in the 1-shot task by 3.5\%, while 5-shot remains similarly competitive. 
% A possible reason for such experimental results is that unlike SS-100, Kinetics-100 has descriptions that are not very descriptive of the visual details of the action scene. Moreover, the Something-Something-V2~\cite{S2Sv2Goyal} dataset is highly fine-grained, with many similar actions differentiated only in subtle ways. Kinetics, on the other hand, is a very coarse dataset
% with low semantic overlap among categories.

%% ICCV VERSION
% As it can be observed in Table~\ref{tab:main_results}, we achieve state-of-the-art-results in 7 out of 8 standard benchmark metrics across the four tested datasets with both variants ResNet-34 and ResNet-50. Notably, our model does not decrease its performance considerably with a smaller backbone and achieves outstanding results in both families of datasets, even in EK-92, where it has to handle spontaneous descriptions. Likewise, our model exceeds the TSN++ transductive, which shows the relevance of using the textual descriptions to modulate the network and make a transductive inference. 
% The TSN~\cite{TSN}, our backbone, has only a weak temporal modeling capacity. This is in sharp contrast to TAM~\cite{Cao_2020_TAM} and ARN~\cite{zhang2020fewshot} which are specially designed to capture temporal information. Despite these disadvantages, our method is able to outperform strong alternatives and baselines. Critically, on SS-100, EK-92, and MetaUCF-101, our TNT model outperforms the best previous result by around 8\% in the 5-shot and 1-shot tasks. Alternatively, on Kinetics-100, TNT beats the best baseline, the TAM model, in the 1-shot task by 3.5\%, while in 5-shot, the result remains similarly competitive. 
% A possible reason for such experimental results is that, unlike MetaUCF-101, Kinetics-100 has significantly fewer training instances.


%Surprisingly, our TNT model without any video pre-training, nor long-term temporal modeling, just with a backbone initialize with ImageNet and adapted by the semantic information of action descriptions in the support set $\supportset$, achieves results almost equal to the state-of-the-art in the 5-shot task and even better in the 1-shot task on both data sets. This demonstrates the power of the semantic information of action descriptions to adapt and enrich the video embedding and improve the prototypes in a transductive setting.
% \victor{It is unclear how one can conclude the following claim from the results in Table 2.} Moreover, our results support the usefulness of the transductive inference itself to overcome the lack of data in a few-shot scenario. 

% Likewise, we observed that even with a backbone pre-trained on ImageNet, we achieved results almost equal to the state-of-the-art in the 5-shot task and even better in the 1-shot task on both data sets, with a smaller backbone. Indeed, by increasing the backbone capacity using the ResNet-50 as \cite{Cao_2020_TAM}, we managed to improve TAM \cite{Cao_2020_TAM} results considerably without explicitly modeling long-term temporal relationships or pre-training on base classes. This demonstrates the effectiveness of the semantic information in action descriptions to modulate the video embedding to each task and improve the prototypes in a transductive setting.

% \begin{table}[t]
% \begin{center}
% \caption{\textbf{Ablation study results} in the validation set.
% We consider: a Video-conditioned Networks with Inductive (VNI) and Transductive (VNT) inference, Text-conditioned Networks with Inductive (TNI) and Transductive (TNT) inference, and the TSN++ baseline.
% } %title of the table
% \resizebox{8cm}{!}{%
%     \begin{tabular}{cccccccc} % creating eight columns
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{\bf Model}} &\multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}{\bf Inference} \\ {\bf Type} \end{tabular}}} &\multicolumn{2}{c}{\bf Task Encoder} & \multicolumn{2}{c}{\bf Kinetics-100} & \multicolumn{2}{c}{\bf SS-100} 
%     \\\cmidrule{3-8} 
%          & & \multicolumn{1}{c}{\bf Video} & \multicolumn{1}{c}{\bf Text} &  \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} & \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} \\
%     \midrule
%     TSN++ & Inductive & \xmark & \xmark & 
%     \begin{tabular}[c]{@{}c@{}}69.11 \\ \pm 1.69 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}81.64 \\ \pm 0.96 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}	35.72 \\ \pm 1.37 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}49.4 \\ \pm 1.24 \end{tabular}
%     \\\midrule
%     VNI & Inductive & \cmark & \xmark & 
%     \begin{tabular}[c]{@{}c@{}}71.23 \\ \pm 1.60 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}86.88 \\ \pm 0.95 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}	33.53 \\ \pm 1.07 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}50.51 \\ \pm 1.30 \end{tabular}
%     \\\midrule
%     TNI & Inductive &\xmark & \cmark & 
%     \begin{tabular}[c]{@{}c@{}}72.16 \\ \pm 1.60 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}\textbf{87.30} \\ \pm 1.06 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}34.27 \\ \pm 1.24 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}56.21 \\ \pm 1.22 \end{tabular}
%     \\\midrule
%     VNT & Transd. & \cmark & \xmark & \begin{tabular}[c]{@{}c@{}}76.37 \\ \pm 1.56 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}85.90 \\ \pm 1.09 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}41.5 \\ \pm 1.53 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}56.60 \\ \pm 1.23 \end{tabular}
%     \\\midrule
%     TNT & Transd. & \xmark & \cmark &
%     \begin{tabular}[c]{@{}c@{}}\textbf{76.40} \\ \pm 1.45 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}86.30 \\ \pm 1.03 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}\textbf{47.98} \\ \pm 1.41 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}\textbf{60.18} \\ \pm 1.21 \end{tabular}
%     \\
%     \bottomrule
%     \end{tabular}}
%     \vspace{-20pt}
% \label{tab:ablations_val}
% \end{center}
% \end{table}

%%%%%%%%%%%%%%%%%%% ICCV21 FORMAT %%%%%%%%%%%%%%%%%%%%%
% \begin{table}[b]
% \begin{center}
% \caption{\textbf{Ablation study results} in the validation set.
% We consider: a Video-conditioned Networks with Inductive (VNI) and Transductive (VNT) inference, Text-conditioned Networks with Inductive (TNI) and Transductive (TNT) inference, the TSN++ baseline, and the TSN-AT baseline based on \cite{BateniSimpleCNAPS, liu2020prototype}.
% } %title of the table
% \resizebox{8cm}{!}{%
%     \begin{tabular}{cccccc} % creating eight columns
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{\bf Model}} &\multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}{\bf Inference} \\ {\bf Type} \end{tabular}}} &\multicolumn{2}{c}{\bf Task Encoder} & \multicolumn{2}{c}{\bf SS-100} 
%     \\\cmidrule{3-6} 
%          & & \multicolumn{1}{c}{\bf Video} & \multicolumn{1}{c}{\bf Text} &
%          \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} \\
%     \midrule
%     TSN++ & Inductive & \xmark & \xmark & $35.72 \pm 1.37$ &  $49.4 \pm 1.24$
%     \\
%     TSN-AT & Transd &\cmark & \xmark & 
%     $42.20 \pm 1.43$ & $57.68 \pm 1.37$
%     \\\midrule
%     VNI & Inductive & \cmark & \xmark & 
% 	$33.53 \pm 1.07$ & $50.51  \pm 1.30$ 
%     \\
%     TNI & Inductive &\xmark & \cmark & 
%     $34.27 \pm 1.24$ & $56.21 \pm 1.22$
%     \\
%     VNT & Transd. & \cmark & \xmark & $41.5\pm 1.53$ &  $56.60 \pm 1.23$
%     \\
%     TNT & Transd. & \xmark & \cmark & $\textbf{47.98} \pm 1.41$ & $\textbf{60.18} \pm 1.21$
%     \\
%     \bottomrule
%     \end{tabular}}
% \label{tab:ablations_val}
% \end{center}
% \end{table}

\begin{table}
\centering
\resizebox{11cm}{!}{
\begin{tabular}{cc}
\bmvaHangBox{
\begin{tabular}{cccccc} % creating eight columns
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\bf Model}} &\multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}{\bf Inference} \\ {\bf Type} \end{tabular}}} &\multicolumn{2}{c}{\bf Task Encoder} & \multicolumn{2}{c}{\bf SS-100} 
    \\\cmidrule{3-6} 
         & & \multicolumn{1}{c}{\bf Video} & \multicolumn{1}{c}{\bf Text} &
         \multicolumn{1}{c}{\bf 1-shot} & \multicolumn{1}{c}{\bf 5-shot} \\
    \midrule
    TSN++ & Inductive & \xmark & \xmark & $35.72 \pm 1.37$ &  $49.4 \pm 1.24$
    \\
    T-TSN+CNAPS & Transd &\cmark & \xmark & 
    $42.20 \pm 1.43$ & $57.68 \pm 1.37$
    \\\midrule
    VNI & Inductive & \cmark & \xmark & 
	$33.53 \pm 1.07$ & $50.51  \pm 1.30$ 
    \\
    TNI & Inductive &\xmark & \cmark & 
    $34.27 \pm 1.24$ & $56.21 \pm 1.22$
    \\
    VNT & Transd. & \cmark & \xmark & $41.5\pm 1.53$ &  $56.60 \pm 1.23$
    \\
    TNT & Transd. & \xmark & \cmark & $\textbf{47.98} \pm 1.41$ & $\textbf{60.18} \pm 1.21$
    \\
    \bottomrule
    \end{tabular}
} & \bmvaHangBox{
\includegraphics[scale=0.45]{images/numQuerySamples.pdf}
}
\end{tabular}
}
% \captionlistentry[table]{A table beside a figure}
% \captionsetup{labelformat=andtable}
\caption{(Left) \textbf{Ablation study results in the validation set.} We consider: a Video-conditioned Networks with Inductive (VNI) and Transductive (VNT) inference, Text-conditioned Networks with Inductive (TNI) and Transductive (TNT) inference, the TSN++ baseline, and the T-TSN+CNAPS baseline based on \cite{BateniSimpleCNAPS, liu2020prototype}.} 
\label{tab:ablation_studies}
\vspace{-1mm}
\captionof{figure}{
(Right) \textbf{Sensitivity analysis to the number of query set samples.} Model performance in the 5-way, 5-shot task for different B size.
}
\vspace{-4mm}
\label{fig:ablation_studies}
\end{table}

\noindent\textbf{Ablation Study.} We analyze the impact of our proposed text encoder and transductive inference approach. To this end, we train and evaluate our model with two different task encoders (text and video) and two inference approaches (Inductive and Transductive). Specifically, we consider video-conditioned networks with inductive ({\bf VNI}) and transductive ({\bf VNT}) inference; and text-conditioned networks with inductive ({\bf TNI}) and transductive ({\bf TNT}) inference. The video-based conditioner module consists of a C3D model with a Conv-4-64 backbone to extract significant spatio-temporal information at low computational cost \cite{zhang2020fewshot}, see Fig.~\ref{fig:encoders_dynaMod}-b. Moreover, we consider the TSN++ \cite{Cao_2020_TAM} as our primary baseline, which is purely based on \cite{TSN} and inductive prototypical learning. For a fair comparison, we also implement T-TSN+CNAPS, a variant of TSN++ with modulation \cite{BateniSimpleCNAPS} and transductive inference based on label propagation \cite{liu2020prototype}. Table \ref{tab:ablation_studies} shows our results. All the results are computed in the validation set using the same visual backbone model (ResNet-34).

It is important to note that feature encoder adaptation generates a substantial increase in model performance with regard to the TSN++ baseline across all evaluation modalities. This is generally true for both the VNI and TNI models. Crucially, the TNI model yields a performance gain of 6\% and 1\% in  5-shot and 1-shot tasks on the SS-100 over VNI, respectively. Likewise, there is a further performance increase, especially in the 1-shot task when the dynamic module is included to perform a transductive inference (TNT and VNT). Interestingly, the 1-shot task is the most data-deprived testing set-up, which speaks positively about the effectiveness of our transductive model. It should be noted that our TNT model outperforms the T-TSN+CNAPS and VNT models by a large margin on both 5-shot and 1-shot tasks. This proves the relevance of using textual descriptions to modulate or contextualize the video feature encoder and improve the class prototypes in a transductive approach.

%%%%%%%%%%%%%%%%%% ICCV Version %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% For our ablation study, we start from the publicly available TSN++, which is a competitive FSL baseline method.
% TSN++ is based purely on TSN feature extraction and cosine-distance prototypical learning, as described in~\cite{Cao_2020_TAM}. 
% For fair comparison, we also implement T-TSN+CNAPS, a few-shot variant of TSN++ with modulation modules \cite{BateniSimpleCNAPS} and transductive inference \cite{liu2020prototype}.
% All the reported results were computed from the same visual backbone model (ResNet-34) and hence rendering a fair comparison.
% %In this section, ablations studies were carried out to determine the effectiveness of each part of our final model. 
% Specifically, we analyze the impact of our proposed text encoder and transductive inference modules in the overall model performance. 
% To this end, we train and evaluate our model with two different task encoders (text and video) and two inference approaches (Inductive and Transductive). We consider video-conditioned networks with inductive ({\bf VNI}) and transductive ({\bf VNT}) inference; and text-conditioned networks with inductive ({\bf TNI}) and transductive ({\bf TNT}) inference. 
% The video-based conditioner module consists of a C3D model with a Conv-4-64 backbone to extract significant spatio-temporal information at a low enough computational cost \cite{zhang2020fewshot}, see Fig.~\ref{fig:encoders_dynaMod}-b. Table \ref{tab:ablation_studies} renders the comparison of the ablation study.
% % To this end, we train and evaluate our model with two different types of task encoders. We evaluate video-based (VNT) and text-based (TNT) conditional encoders. 
% % The video-based conditioner module consists of a C3D model with a Conv-4-64 backbone to extract significant spatio-temporal relation at a low enough computational cost \cite{zhang2020fewshot}, see Fig.~\ref{fig:video_encoder}.
% % Results of this ablation study are collected in Table \ref{tab:ablations_val}.

% From Table~\ref{tab:ablation_studies}, we observe that feature encoder adaptation generates a substantial increase in model performance with regard to the TSN++ baseline model across all evaluation modalities.
% This is generally true for both the VNI and TNI models.
% Crucially, the TNI model yields a performance gain of 6\% and 1\% in  5-shot and 1-shot tasks on the SS-100 over VNI, respectively. 
% % Following our result from the previous section, conclusions are stronger for the SS-100 data. This is clearly due to poorer textual action descriptions in Kinetics-100 class labels.

% For the case of including the dynamic module, the use of a transductive inference further increases performance, especially in the 1-shot task, on both models (TNT and VNT). 
% Interestingly, the 1-shot task is the most data-deprived testing set-up, which speaks positively about the effectiveness of our transductive model. It is important to note that our TNT model outperforms the T-TSN+CNAPS baseline and VNT by a large margin on both 5-shot and 1-shot tasks. This proves the relevance of using the textual descriptions to modulate the video feature encoder and improve the class prototypes in a transductive approach.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%It is also important to note that on SS-100, using the semantic information of the action descriptions to perform the transductive inference, the model performance grows compared to that obtained using the visual information by approximately 6\% and 4\% for the 1-shot and 5-shot tasks, respectively.

% %=========================
% \begin{figure}[ht]
% \centering
% \subfloat[My first picture]{\label{fig:mdleft}{\includegraphics[width=0.8\linewidth]{images/numQuerySamples.pdf}}}\hfill
% \subfloat[My second picture]{\label{fig:mdright}{\includegraphics[width=0.8\linewidth]{images/numQuerySamples.pdf}}}
% \caption{My two big pictures}
% \label{fig:subfigures}
% \end{figure}
% %===========================

% %====== ICCV21 FORMAT ==============
% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.8\linewidth]{images/numQuerySamples.pdf}
% \caption{
% \textbf{Sensitivity analysis to the number of query set samples.} Model performance in the validation set in the 5-way, 5-shot task for different B size. %The model was trained for this task with B=10.
% % \vspace{-0.1cm}
% }
% \label{fig:numQuerySamples}
% \end{figure}

\noindent\textbf{Effect of Query Set Size.}
We assess the TNT model sensitivity to the number of instances in the query set. This study can be observed in Fig. \ref{fig:ablation_studies}. 
We evaluate our model trained on SS-100 in the 5-way, 5-shot task with $B=50$, increasing the value of $B$ from 5 to 100.
%Our model was pretrained on SS-100 in the 5-way, 5-shot task with ImageNet pretraining and $B = 50$. 
Model performance increases until the number of query samples $B=50$ after which it remains almost constant. We hypothesize that this is due to a saturation point on the amount of extra information that can be extracted from query samples. %to get the best class prototypes that our model can. 
%Likewise, if we decrease the size of $\mathcal{Q}$ the model performance is affected in the same way.

We also conduct qualitative evaluations to demonstrate how our model works and the relevance of using textual descriptions to modulate the visual feature encoder and perform a transductive inference. They are shown in the supplementary material.

\noindent\textbf{Visualization of Class Activation Maps.}
An important aspect of our proposed method is its ability to adapt the feature backbone to a particular task. We are interested in verifying the effect of our proposed text-conditioned module in video samples. To study the influence of FiLM layers to modulate the TSN network using semantic information from textual action descriptions, we analyze the class activation mapping (CAM) for the cases with and without employing the FiLM layers. We use our TNT model trained on SS-100 for the 5-shot 5-way task. Fig.~\ref{fig:visulizations}-a shows the visualization obtained for one test sample after applying our TNT model with and without FiLM layers following the Grad-CAM \cite{grad_cam} approach. 

As it can be seen, the TNT model manages to exploit relevant cues from the support textual descriptions. In this example, our FiLM-ed model activations are located in appropriate regions for the action ``Pouring water out of bottle''. Of particular interest, it seems that the effect of our text-conditioned features is to allow the underlying model to focus on the scene elements that matter the most for the particular query sample. This is, in this sample, the bottle and the pouring water. Meanwhile, the model with no FiLM layers tends to attend irrelevant regions. This arguably has effects in a diminished capacity for fine-grained classification.
In general, we found that the conditioning process, based on the textual action descriptions, enables the network to obtain better video features for specific tasks.

% % \begin{figure}[!t]
% % \centering
% % \includegraphics[width=\linewidth]{images/attn_img_new.pdf}
% % \caption{\textbf{Visualization of dynamic module output for the class: ``Digging something out of something".} Top-3 relevant unlabeled samples for the class in a 5-way 5-shot task. The darkest color indicates the most important sample.
% % }
% % \label{fig:att_example}
% % \end{figure}

\noindent\textbf{Dynamic Module Inspection.}
To assess the transductive capabilities of our model, we closely study the proposed dynamic module.  We exploit our SS-100-trained TNT model in the 5-way 5-shot setting. For this experiment, we directly observe the values of the relevance weight matrix $\mathbf{W}$, which can be easily interpreted. 
Indeed, they encode how relevant is each one of the query set videos to the semantic class embedding obtained by textual descriptions of the support set $\textbf{E}_{class}^{\mathcal{T}}$.
Fig.~\ref{fig:visulizations}-b shows the three most related videos from the query set $\queryset$ to the ``digging something out of something'' class. The text-driven class representation is obtained by averaging the semantic embedding of all sampled descriptions for this class in the support set. These descriptions are shown at the bottom of the figure.
Furthermore, in this figure, we present a heatmap in which darker color means greater relevance of the query video sample to the actual support set description.
Interestingly, the top three most related videos from the query set are the ones that also belong to the class ``digging something out of something''.
This example demonstrates that our dynamic module can leverage the semantic information of textual action descriptions to augment the support set samples with unlabeled samples from the query set. 
This behavior of our model is essential to improve class prototypes and alleviate the problem of low training data. 

\begin{figure}
\centering
\begin{tabular}{cc}
\resizebox{5.5cm}{!}{
\bmvaHangBox{
\includegraphics[scale=0.5]{images/CAM.pdf}
}} & \resizebox{5.5cm}{!}{
\bmvaHangBox{
\includegraphics[scale=0.4]{images/attn_img_new.pdf}
}}\\(a) & (b)
\end{tabular}
\caption{
\textbf{Visualizations.} (a) We take our model pre-trained on SS-100 in the 5-shot and 5-way task and analyze the changes of its CAMs with and without using the FiLM layers before the last average pooling layer of the ResNet. (b) Top-3 relevant unlabeled samples for the class in a 5-way 5-shot task. The darkest color indicates the most important sample.
}
\label{fig:visulizations}
\end{figure}

% \begin{table}[h]
% \caption{\textbf{Ablation studies results.} We compare our method's performance with two kinds of Task Encoder (Text and Video) and analyze the effect of the Dynamic Module.} %title of the table
% \centering % centering table
% \resizebox{8.3cm}{!}{%
%     \begin{tabular}{c|cc|cc} % creating eight columns
%     \hline
%     \multicolumn{1}{c|}{\multirow{2}{*}{Model}}&\multicolumn{2}{c|}{Kinetics} & \multicolumn{2}{c}{S2S-V2} 
%     \\\cline{2-5} 
%          & \multicolumn{1}{c}{1-shot} & \multicolumn{1}{c|}{5-shot} & \multicolumn{1}{c}{1-shot} & \multicolumn{1}{c}{5-shot} \\
%     \hline
%     TSN++ \cite{Cao_2020_TAM} & 64,5 \% & 77,9 \% & 33,6 \% & 43,0 \% 
%     \\\hline
%     TSNFilm + Video Encoder & 
%     \begin{tabular}[c]{@{}c@{}}67,71\% \\ \pm 0,24 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}83,97\% \\ \pm 0,18 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}29,86\% \\ \pm 0,15 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}44,85\% \\ \pm 0,18 \end{tabular}
%     \\\hline
%     \begin{tabular}[c]{@{}c@{}}TSNFilm + Video Encoder \\ + Dynamic Module \end{tabular} & \begin{tabular}[c]{@{}c@{}}71,86\% \\ \pm 0,24 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}83,93\% \\ \pm 0,17 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}34,29\% \\ \pm 0,18 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}47,13\% \\ \pm 0,19 \end{tabular}
%     \\\hline
%     TSNFilm + Text Encoder & 
%     \begin{tabular}[c]{@{}c@{}}68,87\% \\ \pm 0,24 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}83,78\% \\ \pm 0,18 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}31,38\% \\ \pm 0,17 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}46,51\% \\ \pm 0,18 \end{tabular}
%     \\\hline
%     \begin{tabular}[c]{@{}c@{}}TSNFilm + Text Encoder \\ + Dynamic Module \end{tabular} & 
%     \begin{tabular}[c]{@{}c@{}}\textbf{74,92\%} \\ \pm 0,24 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}\textbf{84,14\%} \\ \pm 0,17 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}\textbf{43,17\%} \\ \pm 0,19 \end{tabular} &  \begin{tabular}[c]{@{}c@{}}\textbf{51,43\%} \\ \pm 0,19 \end{tabular}
%     \\
%     \bottomrule
%     \end{tabular}}
% \label{tab:ablations}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%% Supplementary material
% \begin{figure}
% \centering
% \resizebox{11cm}{!}{
% \begin{tabular}{cc}
% \bmvaHangBox{
% \includegraphics[scale=0.5]{images/CAM.pdf}
% \label{fig:filmFunction}
% } & \bmvaHangBox{
% \includegraphics[scale=0.4]{images/attn_img_new.pdf}
% \label{fig:att_example}
% }\\(a) & (b)
% \end{tabular}
% }
% \caption{
% \textbf{Visualizations.} (a) We take our model pre-trained on SS-100 in the 5-shot and 5-way task and analyze the changes of its CAMs with and without using the FiLM layers before the last average pooling layer of the ResNet. (b) Top-3 relevant unlabeled samples for the class in a 5-way 5-shot task. The darkest color indicates the most important sample.
% }
% \label{fig:visulizations}
% \end{figure}

% % \begin{figure}[!t]
% % \centering
% % \includegraphics[width=0.9\linewidth]{images/CAM.pdf}
% % \caption{\textbf{Visualization of the class activation map (CAM).}  We take our model pre-trained on SS-100 in the 5-shot and 5-way task and analyze the changes of its CAMs with and without using the FiLM layers before the last average pooling layer of the ResNet.
% % }
% % \label{fig:filmFunction}
% % \end{figure}

% \noindent\textbf{Visualization of Class Activation Maps.}
% An important aspect of our proposed method is its ability to adapt the feature backbone to the particular sampled task at any given point. We are interested in verifying the effect
% of our proposed text-conditioned module in actual video samples.
% %For this reason, we focus on exploring how those mechanisms are working qualitatively. 
% To study the influence of FiLM layers to modulate the TSN network using semantic information from textual action descriptions, we analyze the class activation mapping (CAM) for the cases with and without employing the FiLM layers. We use our TNT model trained on SS-100 for the 5-shot 5-way task. % with an ImageNet pre-training because we want to observe how the FiLM mechanism works in a network without any previous specialization in the particular problem.  
% Fig.~\ref{fig:visulizations}-a shows the visualization obtained for one test sample after applying our TNT model with and without FiLM layers following the Grad-CAM \cite{grad_cam} approach. 

% As it can be seen, the TNT model manages to exploit relevant cues from the textual descriptions in the support set. %the semantic information to focus on what is really important to understand the video. 
% In this specific example, our FiLM-ed model activations are located in appropriate regions for the action ``Pouring water out of bottle''. 
% Of particular interest, it seems that the effect of our text-conditioned features is to allow the underlying model to focus on the scene elements that matter the most for the particular query sample. This is, in this sample, the bottle and the pouring water.
% %such as the bottle and the one that shows the water pouring. 
% Meanwhile, the model with no FiLM layers tends to attend irrelevant regions. This arguably has effects in diminished capacity for fine-grained classification.
% In general, we found that the conditioning process, based on the textual action descriptions, enables the network to obtain better video features for specific tasks.

% % \begin{figure}[!t]
% % \centering
% % \includegraphics[width=\linewidth]{images/attn_img_new.pdf}
% % \caption{\textbf{Visualization of dynamic module output for the class: ``Digging something out of something".} Top-3 relevant unlabeled samples for the class in a 5-way 5-shot task. The darkest color indicates the most important sample.
% % }
% % \label{fig:att_example}
% % \end{figure}

% \noindent\textbf{Dynamic Module Inspection.}
% To assess the transductive capabilities of our model, we closely study the proposed dynamic module. 
% We exploit our SS-100-trained TNT model in the 5-way 5-shot setting. 
% For this experiment, we directly observe the values of the relevance weight matrix $\mathbf{W}$. The values of such matrix are in fact easily interpreted. 
% Indeed, they encode how relevant is each one of the query set videos to the semantic class embedding obtained by textual descriptions of the support set $\textbf{E}_{class}^{\mathcal{T}}$.
% Fig.~\ref{fig:visulizations}-b shows the three most related videos from the query set $\queryset$ to the ``digging something out of something'' class. The text-driven class representation is obtained by averaging the semantic embedding of all sampled descriptions for this class in the support set. These descriptions are shown at the bottom of the figure.
% Furthermore, in this figure, we present a heatmap in which darker color means greater relevance of the query video sample to the actual support set description.
% Interestingly, the top three most related videos from the query set are the ones that also belong to the class ``digging something out of something''.
% This example demonstrates that our dynamic module can leverage the semantic information of textual action descriptions to augment the support set samples with unlabeled samples from the query set. 
% This behavior of our model is essential to improve class prototypes and to alleviate the problem of low training data. 
